TED: A Tolerant Edit Distance for Segmentation Evaluation

In this paper, we present a novel error measure to compare a segmentation against ground truth. This measure, which we call Tolerant Edit Distance (TED), is motivated by two observations: (1) Some errors, like small boundary shifts, are tolerable in practice. Which errors are tolerable is application dependent and should be a parameter of the measure. (2) Non-tolerable errors have to be corrected manually. The time needed to do so should be reflected by the error measure. Using integer linear programming, the TED finds the minimal weighted sum of split and merge errors exceeding a given tolerance criterion, and thus provides a time-to-fix estimate. In contrast to commonly used measures like Rand index or variation of information, the TED (1) does not count small, but tolerable, differences, (2) provides intuitive numbers, (3) gives a time-to-fix estimate, and (4) can localize and classify the type of errors. By supporting both isotropic and anisotropic volumes and having a flexible tolerance criterion, the TED can be adapted to different requirements. On example segmentations for 3D neuron segmentation, we demonstrate that the TED is capable of counting topological errors, while ignoring small boundary shifts.

==> funkey/commands.tex <==
% This file provides some helpful macro commands.

\usepackage{todonotes}
\usepackage{xspace}

% todo-notes with a special color
\def\idea#1{{\todo[color=yellow!90!white]{#1}}\xspace}
\def\note#1{{\todo[color=orange!90!white]{#1}}\xspace}

% evaluate a mathematical expression #2 and assign the result to macro #1
\def\mathlet#1#2{\pgfmathparse{#2}\let#1\pgfmathresult}

% mark text as draft
\newenvironment{draft}{\color{red}}{}

% include a part of an image
\def\includetrimmed#1#2#3#4#5{%
  \includegraphics[%
    width=\samplewidth,%
    height=\sampleheight,%
    trim=#1px #2px #3px #4px,%
    clip]%
    {#5}%
}
\def\includesubimage#1#2#3#4#5{%
  \mathlet\l{#1}%
  \mathlet\t{#2}%
  \mathlet\r{\totalwidth-#3-#1}%
  \mathlet\b{\totalheight-#4-#2}%
  \includetrimmed{\l}{\b}{\r}{\t}{#5}%
}

% include files in a directory relative to current directory
\def\currentdir{.}%
\def\linput#1#2{%
  \begingroup%
  \edef\currentdir{\currentdir/#1}%
  \input{\currentdir/#2}%
  \endgroup%
}%


==> funkey/math.tex <==
% This file provides definitions of mathematical operators, symbols, and theorem 
% environments.


% defining equality
\newcommand{\define}{\stackrel{\text{\tiny def}}{=}}

% argmin, argmax
\newcommand{\argmin}[1]{\mathop{\arg\min}_{#1}\hspace{0.5em}}
\newcommand{\mmin}[1]{\mathop{\min}_{#1}\hspace{0.5em}}
\newcommand{\argmax}[1]{\mathop{\arg\max}_{#1}\hspace{0.5em}}
\newcommand{\mmax}[1]{\mathop{\max}_{#1}\hspace{0.5em}}

% const
\newcommand\const{\text{const}}

% transpose and inverse
\newcommand{\trans}[0]{{\sf T}}
\newcommand\inv{{-1}}

% annotations in equations
\newcommand{\annotation}[1]{& \text{{\small{#1}}}}

% function names
\newcommand\gauss{\mathcal{N}}

% ILP
%
% Usage:
%
% \beginilp
%   \objective{\
\def\beginilp{%
  \makeatletter
  \global\let\ilp@firstconstraint 0
  \global\def\ilp@name{}
  \makeatother
  % [name]{min,s.t.}[spacer]{objective,lhs}[rel][rhs][spacer][qualifier]
  \begin{IEEEeqnarray}{lr?rCl"l}
}
\def\name#1{%
  \makeatletter
  \global\def\ilp@name{#1:\;\;\;\;}
  \makeatother
}
\def\objective#1#2{%
  \makeatletter
  \global\let\ilp@firstconstraint 1
  \ilp@name
  \makeatother
  &
  #1
  &
  \IEEEeqnarraymulticol{4}{l}{#2}
}
\def\objectivecont#1{%
  \\
  &
  &
  \IEEEeqnarraymulticol{4}{l}{#1}
  \nonumber
}
\def\constraint#1#2#3#4{%
  \\
  &
  \makeatletter
  \if\ilp@firstconstraint 1 \text{s.t.} \fi
  \global\let\ilp@firstconstraint 0
  \makeatother
  &
  #1
  &
  #2
  &
  #3
  &
  #4
}
\def\endilp{%
  \end{IEEEeqnarray}
}


==> funkey/notation.tex <==
\usepackage{xifthen}

% isin version that expands its first argument
\newcommand*{\isinxp}[2]{\expandafter\isin\expandafter{#1}{#2}}

\newcommand{\mbb}[1]{{%
\ifthenelse{\isinxp{#1}{abcdefghijklmnopqrstuvxyz}}%
  {{\mathbf #1}}%
  {\boldsymbol #1}%
}}
\newcommand{\mup}[1]{{%
\ifthenelse{\isin{#1}{abcdefghijklmnopqrstuvxyzABCDEFGHIJKLMNOPQRSTUVXYZ}}%
  {\text{#1}}%
  {#1}%
}}

% vector
\newcommand{\vct}[1]{\protect\mbb{#1}}
% matrix
\newcommand{\mat}[1]{#1}
% set
\newcommand{\set}[1]{\protect\mbb{#1}}
% super-set
\newcommand{\sset}[1]{\boldsymbol{\mathcal{#1}}}
% random variable
\newcommand{\ran}[1]{#1}
% function
\newcommand{\fun}[1]{\mathrm{#1}}

% whole numbers
\newcommand{\whole}[0]{\mathbb{Z}}
% real numbers
\newcommand{\real}[0]{\mathbb{R}}
% natural numbers
\renewcommand{\natural}[0]{\mathbb{N}}

% abbreviations
\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}


==> funkey/tables.tex <==
% this file provides useful extensions to pgfplotstable:
%
% styles (found on stackexchange by user Jake):
%
%   highlight col max
%   highlight col min
%   highlight row max
%   highlight row min
% 
%   Usage:
%
%     \pgfplotstabletypeset[
%       highlight row max={<data>}{<row number>}
%     }{<data>}
%
%     or
%
%     \pgfplotstabletypeset[
%       highlight col max={<data>}{<column name>}
%     }{<data>}

\usepackage{pgfplotstable}
\usepackage{booktabs}
\usepackage{colortbl}

\newcommand{\findmax}[3]{%
    \pgfplotstablevertcat{\datatable}{#1}%
    \pgfplotstablecreatecol[%
    create col/expr={%%
    \pgfplotstablerow%
    }]{rownumber}\datatable%
    \pgfplotstablesort[sort key={#2},sort cmp={float >}]{\sorted}{\datatable}%%
    \pgfplotstablegetelem{0}{rownumber}\of{\sorted}%%
    \pgfmathtruncatemacro#3{\pgfplotsretval}%
    \pgfplotstableclear{\datatable}%
}%

\newcommand{\findmin}[3]{%
    \pgfplotstablevertcat{\datatable}{#1}%
    \pgfplotstablecreatecol[%
      create col/expr={%
    \pgfplotstablerow%
    }]{rownumber}\datatable%
    \pgfplotstablesort[sort key={#2},sort cmp={float <}]{\sorted}{\datatable}%
    \pgfplotstablegetelem{0}{rownumber}\of{\sorted}%%
    \pgfmathtruncatemacro#3{\pgfplotsretval}%
    \pgfplotstableclear{\datatable}%
}%

\pgfplotstableset{
  highlight content/.style={
    postproc cell content/.append style={
      @cell content/.add={$\bf}{$},
    }
  },
  highlight min content/.style={
    highlight content
  },
  highlight max content/.style={
    highlight content
  },
}

\pgfplotstableset{
    highlight col max/.code 2 args={
        \findmax{#1}{#2}{\maxval}
        \edef\setstyles{\noexpand\pgfplotstableset{
                every row \maxval\noexpand\space column #2/.style={
                    highlight max content
                }
            }
        }\setstyles
    },
    highlight col min/.code 2 args={
        \findmin{#1}{#2}{\minval}
        \edef\setstyles{\noexpand\pgfplotstableset{
                every row \minval\noexpand\space column #2/.style={
                    highlight min content
                }
            }
        }\setstyles
    },
    highlight row max/.code 2 args={
        \pgfmathtruncatemacro\rowindex{#2-1}
        \pgfplotstabletranspose{\transposed}{#1}
        \findmax{\transposed}{\rowindex}{\maxval}
        \edef\setstyles{\noexpand\pgfplotstableset{
                every row \rowindex\space column \maxval\noexpand/.style={
                    highlight max content
                }
            }
        }\setstyles
    },
    highlight row min/.code 2 args={
        \pgfmathtruncatemacro\rowindex{#2-1}
        \pgfplotstabletranspose{\transposed}{#1}
        \findmin{\transposed}{\rowindex}{\maxval}
        \edef\setstyles{\noexpand\pgfplotstableset{
                every row \rowindex\space column \maxval\noexpand/.style={
                    highlight min content
                }
            }
        }\setstyles
    },
}

\makeatletter%
\long\def\pgfplotstabletypeset@opt@collectarg[#1]#2{%
    \pgfplotstable@isloadedtable{#2}%
        {\pgfplotstabletypeset@opt@[#1]{#2}}%
        {\pgfplotstabletypesetfile@opt@[#1]{#2}}%
}%
\makeatother%


==> funkey/theorems.tex <==
% theorem environments

\usepackage{amsmath}
\usepackage{framed}
\usepackage[framed,thmmarks,amsmath]{ntheorem}

% general theorem style
\theoremstyle{plain}
\theorembodyfont{}
\def\theoremframecommand{\fcolorbox{black}{gray!20!white}}

\newshadedtheorem{theorem}{Theorem}[section]

\newshadedtheorem{lemma}[theorem]{Lemma}

\newshadedtheorem{proposition}[theorem]{Proposition}

\newshadedtheorem{corollary}[theorem]{Corollary}

\newshadedtheorem{definition}{Definition}[section]

{
\theoremstyle{nonumberplain}
\ifdefined\alternativetheoremsymbol
  \theoremsymbol{\alternativetheoremsymbol}
\else
  \theoremsymbol{\rule{1ex}{1ex}}
\fi
\theoremseparator{:}
\newtheorem{proof}{Proof}[section]
}


==> funkey/tikztension.tex <==
% This is the externalization variant of the tikztension, i.e., the one that 
% should be used to send to journals etc. It assumes that all graphics have been 
% generated in an appropriate format (pdf, ps, or eps) already. This is how you 
% can get rid of the tikz-dependence for publications.
\usepackage{graphics}

% single escape
%
% escapes a single character
\def\sesc#1{%
\if#1.-%   . -> -
\else%
\if#1=-%   = -> -
\else%
\if#1,-%   , -> -
\else%
\if#1/-%   / -> -
\else#1%
\fi%
\fi%
\fi%
\fi%
}

% denotes the end of the sequence to escape
\def\escnull{}

% escapes a sequence that ends with \escnull followed by \escend
\def\esc#1#2\escend{%
\ifx#1\escnull%
\else%
\sesc#1\esc#2\escend%
\fi%
}

% Escapes a string using the replacements in \sesc. Introduces no non-expandable 
% macros, i.e., the result can safely be used for filenames.
\def\escape#1{\esc#1\escnull\escend}

% #1 is the base name of the tikz file
% #2 is a string of PGF keys that are passed to \begin{tikzpicture}. It may 
% contain the special key /tikztension/define that defines empty macros. These 
% can be used as flags in the tikzimage via \ifdefined.
\newcommand{\includetikz}[2][]{%
  \def\graphicname{#2-\escape{#1}}%
  % include externalized graphic
  \includegraphics{\graphicname}%
}%

